Put Your Money Where Your Mouth Is: Evaluating Strategic Planning and Execution of LLM Agents in an Auction Arena

Recent advancements in Large Language Models (LLMs) showcase advanced reasoning, yet NLP evaluations often depend on static benchmarks. Evaluating this necessitates environments that test strategic reasoning in dynamic, competitive scenarios requiring long-term planning. We introduce AucArena, a novel evaluation suite that simulates auctions, a setting chosen for being highly unpredictable and involving many skills related to resource and risk management, while also being easy to evaluate. We conduct controlled experiments using state-of-the-art LLMs to power bidding agents to benchmark their planning and execution skills. Our research demonstrates that LLMs, such as GPT-4, possess key skills for auction participation, such as budget management and goal adherence, which improve with adaptive strategies. This highlights LLMs' potential in modeling complex social interactions in competitive contexts. However, variability in LLM performance and occasional outperformance by simpler methods indicate opportunities for further advancements in LLM design and the value of our simulation environment for ongoing testing and refinement.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Abstract and Section 1
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We set the temperature to 0 for all models. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no societal impact of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3 and Section 4 and Appendix A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/070ethics.tex <==

This auction simulation has the potential to allow and somehow encourage participators acting as bidder agents to lie to each other, for the purpose of being strategic and victorious in an auction game.
This is especially true if advanced auction rules like collaboration and negotiation between bidders are introduced into this auction arena.
Agents developed in such an arena could emerge as calculative, deceptive, greedy, dishonest, and manipulative.


==> sections/080limitations.tex <==

Limited by a research paper, we keep \method to be simple and controllable for a better understanding and evaluation of LLM agents.
For example, we design limited types of item values, the same budget for everyone, only two objectives for bidders, and no autonomy for the auctioneer.
We believe there are numerous combinations of settings that this simulated arena can offer, such as different desires for bidders, personalized item values, etc.
Besides, due to budget limits, we did not experiment with the variety of prompts. 
As with the previous work, we iterated on the selection of input prompts, specifically choosing prompts that encourage participation in the auction.  
However, we clarify that these instruction prompts (Appendix~\ref{appendix:prompt}) only inform the agent of the must-known rules in the auction, rather than telling the agent high-level guidance (e.g., ``you need to save money because there might be more lucrative items later''), or provide some few-shot examples in the prompts. 




==> tables/list_learning.tex <==

\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Human,Bidder, \#1,\#2,\#3,\#4,\#5,GPT-3.5,Claude-Instant-1.2,Claude-2,PaLM-2},
    emphstyle={\bfseries\color{brown}}
}\begin{lstlisting}[caption={Strategic learnings and takeaways from human bidders and LLM-agents after 10 rounds of games in auction arena.},label=lst:human_learning]
Human Bidder #1:
All in all, every bidder has specific strategies or tendencies.
bidder1: Tend to buy nothing
bidder2: Waiting for opportunities, likes to pick up leaks.
bidder3: Most of the time, it is conservative and likes to withdraw, and rarely gives a price exceeding 1.6 times the starting price.
bidder4: Pay more attention to large items of $5000 because it is possible to obtain higher profits. It's easy to withdraw from the initial 1000 small items. If the bidding price exceeds 1.6 times, it is easy to withdraw the bidding.
bidder5: Sometimes it makes sudden decisions and buys goods at irrational prices (buy a $1000 item by more than $10000).
bidder6: Love buying from the beginning, no matter how much the item costs, until the money runs out. 
bidder7: Pay attention to large items of $5000, pick up leaks if the price of $1000-items are below $1600. I bid up the price before bidder6 finished buying. Try to let bidder2&bidder4 get $5000-items with a price higher than $8000 (so the left money is lowwer than $7000 and I can pick the ups of other 5000-items). Generally speaking, 1.5 times the starting price is a dividing line for me to measure whether a product is a good deal.
I think the number of $5000-items and the order in which they appear have a great impact on the strategy of the game. If $5000-items appear later, the previous $1000-items will be easily missed by these models so that I can pick the leaks. If there are more $5000-items, then the variables in the game will become larger and it will be harder for me to control the behavior of other models.

Human Bidder #2:
1. Primarily focus on the four 5k items, keeping at least 8k on hand until at least the penultimate 5k item, to prevent any bidder from buying the 5k item at a low price and making a substantial profit. Each 5k item should be bid up to at least 7k.
2. For the 1k items: Since bidder 6 will continuously increase the price in the auction of the 1k items for profit, it's necessary to compete with them, raising the price to 1700. (Since bidder 6 will also buy 5k items, it's crucial to ensure they don't make too much on the 1k items.)
3. The last few 1k items may be priced over 2k, so don't expect to make a profit from them.

Human Bidder #3:
It is evident that bidder 5 and bidder 6 exhibit a propensity for purchasing items priced at 2000 units, whereas bidder 3 and bidder 2 demonstrate a preference for items priced at 5000 units. Building upon these observations, we can formulate a strategic approach:
Purchase a total of 6 items: 5 priced at 2000 units (with a target price below 1500) and 1 priced at 10000 units (with a target price below 7500).
1. Early Game: Implement a proactive bidding strategy by offering higher prices, such as bidding 3000 for 2000-priced items and 11000 for 10000-priced items. This approach aims to deplete the funds of other players and reduce the likelihood of intense competition in the mid to late game. The primary focus here is on bidders 5 and 6, as bidder 6 frequently engages early in the game.
2. Mid-Game: Concentrate on acquiring 2000-priced items for 1500 units or less and securing 10000-priced items for 7500 units or less. Initiate bidding around 6000 units for 10000-priced items, and if the price exceeds 7500 units, consider abandoning the item. The objective is to encourage other players to purchase items at prices exceeding 7500 units, thereby preventing them from acquiring two 10000-priced items consecutively.
3. Exercise caution when making purchases near the end of the game. Players with remaining funds often engage in continuous bidding, leading to higher prices, particularly for items priced at 2000 units, which may exceed 1800 units.

Human Bidder #4:
In earlier experiments, it was observed that bidders who could start with a bid of 5000 in the later stages often ended up winning. This is because, by the latter stages, many bidders had already spent a significant amount of money and did not have enough left to bid on items with a starting price of 5000. Additionally, given that the order of the items is random, there's a chance that an item priced at 5000 could appear twice, both in the first ten rounds and the last ten rounds of a 20-round auction. Thus, in subsequent tests, the strategy was to drive up the prices in the first ten rounds to deplete the machine bidders' funds. Specifically, human bidder would start by bidding 1.5 times the original price to drive up the costs and then opt out of the following bids. In the last ten rounds, human bidder would engage in bidding, always increasing bid by the minimum increment over the highest previous bid. Using this strategy, human bidder often managed to win items with a starting price of 5000 for a bid of 7500 or less, as well as several items with a starting price of 1000 for 1500 or less.

Human Bidder #5:
I find that language models tend to spend all the money in the first few rounds, and the later bids are much less than the previous ones. From a profit perspective, items worth 2000 generally bring a relatively low profit, so we can spend money on items worth 10000. For items worth 2000, each bid is around 1700, preventing others from getting their money at a low price and consuming their money. For items worth 10000, i bid around 8000 in the first two times. I find other auctioneers usually follow me, which results in others earning less. Afterwards, i can bid for a low price (6500/7000). Following this strategy can usually win!

GPT-4 Bidder:
1. Patience and endurance often pay off, as many winning bids emerge from consistent and steady increases rather than an initial high bid.
2. Understanding the true value of an item is key to determining your maximum bid and avoiding overpayment.
3. Regular participation in the bidding process is crucial. Winners often demonstrate active engagement throughout the auction.
4. Be observant of other bidders' behaviors. Early withdrawals can present opportunities for a winning bid.
5. Avoid 'auction fever,' or the excitement that can lead to overbidding. Stick to your predetermined maximum bid.
6. A significant jump in your bid can deter other bidders but should be within your budget and strategically considered.
7. Don't be discouraged if you're not leading early in the auction. Many winners aren't the early frontrunners.
8. Observing the bidding behavior of others can provide valuable insights to inform your strategy.
9. Be flexible and adaptable in your bidding strategy, ready to revise it based on the actions of other bidders.
10. Maintain financial discipline. Be aware of your budget and do not exceed it.
11. Begin active bidding when the price is within a reasonable range of your valuation. Early active bidding might escalate the prices quickly.
12. Sometimes, holding back and not rushing into bidding can provide valuable insights into other bidders' behaviors.
13. Regularly reassess your strategy during the auction based on the behavior of other bidders and the current highest bid.
14. Winning at an auction does not always mean paying the highest price; sometimes, it's about outlasting the competition and having the last valid bid when others have withdrawn.
15. It's important to not get emotionally attached to an item to avoid bidding beyond its worth or your budget.
16. A successful bidder knows when to fight for an item and when to let it go, understanding that not every item is worth winning at any cost.
17. Understanding the dynamics of an auction and the psychology of other bidders can be more valuable than the financial capacity to bid high.
18. Always have a well-thought-out exit strategy; knowing when to stop is as important as knowing when to bid.

GPT-3.5 Bidder:
1. Setting a reserve price can help ensure that the starting bid is closer to the true value of the item and discourage low initial bids and subsequent withdrawals.
2. Analyzing bidding patterns and strategically increasing bids in small increments can help maintain a competitive advantage.
3. Considering the motivations and strategies of other participants and adjusting bidding strategies accordingly can improve the chances of success.
4. Continuously monitoring the number of active bidders and adjusting strategies as the auction progresses, taking into account decreasing bidding activity and the potential for remaining bidders to withdraw, is important.
5. Evaluating the perceived value of an item and considering it alongside the final hammer price is crucial, as the final price can be influenced by bidding strategies and competitive dynamics among bidders.
6. Anticipating potential bidding dynamics and withdrawals based on outbidding by previous bidders and adjusting strategies accordingly can improve competitiveness.
7. Carefully considering the starting price of an item and its impact on bidder engagement and competition is important, as it can significantly affect bidding activity and the final price.
8. Regularly assessing and adapting bidding strategies based on the behavior and patterns of participants can help inform future decision-making.
9. Implementing bidding increments that encourage competitive bidding while avoiding excessive jumps that can discourage participation is beneficial.
10. Using historical auction data to analyze and understand bidding behavior, identifying trends and patterns, can inform future bidding strategies.

Claude-Instant-1.2 Bidder:
1. Monitor the number of active bidders on each item to assess competition level and determine an appropriate maximum budget that allows winning bids without overpaying.
2. Strategically withdraw counterbidding when only one opponent remains and the price exceeds your maximum budget, rather than unnecessarily increasing bids just to determine the highest bidder.
3. Successively outbidding opponents by small incremental amounts is an effective tactic to win items when within budget, avoiding unnecessarily driving prices much higher through large counterbids against multiple bidders.

Claude-2 Bidder:
1. Identify and track competitors who habitually overbid to exploit their tendencies.
2. Make bold opening bids to test waters, but be ready to withdraw if competition emerges.
3. Bid just enough to stay competitive when facing multiple engaged bidders.
4. Restart stalled bidding below true value if possible to extract better deals.
5. Time bids for maximal impact when competitors seem distracted or disengaged.
6. Withdraw quickly at preset limits to avoid overpaying in the heat of bidding.
7. Cautiously bid on items with little early engagement to get good value.
8. Be willing to incrementally increase bids on coveted items up to your limit.
9. Use small bid bumps to win uncontested items without overpaying.
10. Balance bid amounts based on number of competitors and intensity of engagement.

PaLM-2 Bidder:
1. Bidders often withdraw their bids, so it is important to be prepared to increase your bid if you are interested in an item.
2. The number of bidders and the level of competition can vary significantly from auction to auction, so it is important to be prepared to adjust your bidding strategy accordingly.
3. The starting price of an item is not necessarily indicative of its final sale price.
4. Some bidders may be more willing to pay a higher price for an item than others, so it is important to be aware of the competition and be prepared to adjust your bid accordingly.
5. The true value of an item may not be known until the end of the auction, so it is important to carefully consider your maximum bid before placing it.
6. It is important to have a clear bidding strategy in place before the auction starts, and to stick to it.
\end{lstlisting}

==> tables/main.tex <==
\begin{table}[ht]
\centering
\caption{TrueSkill Scores and Deviations for 20k Models}
\begin{tabular}{lrrr}
\hline
Model & RANDOM & L2M & M2L \\
\hline
gpt-4-1106-preview & 28.77 $\pm$ 2.60 & 29.57 $\pm$ 2.28 & 27.52 $\pm$ 2.50 \\
rule-5 & 29.00 $\pm$ 2.44 & 26.74 $\pm$ 2.12 & 28.43 $\pm$ 2.47 \\
mixtral & 27.79 $\pm$ 2.60 & 25.00 $\pm$ 3.15 & 27.58 $\pm$ 2.65 \\
gemini & 24.76 $\pm$ 2.69 & 25.00 $\pm$ 3.15 & 28.54 $\pm$ 2.56 \\
rule-4 & 31.38 $\pm$ 2.84 & 32.72 $\pm$ 3.50 & 32.27 $\pm$ 2.73 \\
llama-13b & 12.09 $\pm$ 4.05 & 11.94 $\pm$ 4.13 & 12.34 $\pm$ 4.02 \\
open-mistral-7b & 18.53 $\pm$ 2.72 & 18.55 $\pm$ 2.76 & 20.57 $\pm$ 2.47 \\
gpt-3.5-turbo-1106 & 24.07 $\pm$ 2.54 & 21.98 $\pm$ 2.71 & 22.06 $\pm$ 2.43 \\
gpt-4-0613 & 28.87 $\pm$ 2.55 & 25.82 $\pm$ 2.54 & 26.87 $\pm$ 2.61 \\
\hline
\end{tabular}
\end{table}

